Sample complexity of data-driven tuning of model hyperparameters in neural networks with structured parameter-dependent dual function

Modern machine learning algorithms, especially deep learning based techniques, typically involve careful hyperparameter tuning to achieve the best performance. Despite the surge of intense interest in practical techniques like Bayesian optimization and random search based approaches to automating this laborious and compute intensive task, the fundamental learning theoretic complexity of tuning hyperparameters for deep neural networks is poorly understood. Inspired by this glaring gap, we initiate the formal study of hyperparameter tuning complexity in deep learning through a recently introduced data driven setting. We assume that we have a series of deep learning tasks, and we have to tune hyperparameters to do well on average over the distribution of tasks. A major difficulty is that the utility function as a function of the hyperparameter is very volatile and furthermore, it is given implicitly by an optimization problem over the model parameters. To tackle this challenge, we introduce a new technique to characterize the discontinuities and oscillations of the utility function on any fixed problem instance as we vary the hyperparameter; our analysis relies on subtle concepts including tools from differential/algebraic geometry and constrained optimization. This can be used to show that the learning theoretic complexity of the corresponding family of utility functions is bounded. We instantiate our results and provide sample complexity bounds for concrete applications tuning a hyperparameter that interpolates neural activation functions and setting the kernel parameter in graph neural networks.

==> archived_files/previous-case.tex <==
\subsection{Second case: one-dimensional parameter and hyperparameter, single piece, and no boundary function.} 
We now consider the case where there is only one piece function. In particular, we assume that $N = 1$ and $M = 0$. In this case, we first present the following structural result for the function class $\cG$.

% The following arguments in the the proof of that case could help us.
% \begin{assumption} The following arguments are assumed to be true: 
%     \begin{enumerate}
%         \item From Lemma 1.1.a in Dravy's draft, we know the upper-bound for the number of continuous intervals of the functions 
%         $$
%             g^{b_j}_i(\alpha) = \max_{W}f_i(\alpha, W) \quad \text{s.t. } \quad h_j(\alpha, W) = 0.
%         $$
        
%         \item From Lemma 1.1.a in Dravy's draft, in each continuous interval, we know the upper-bound for the number of local maxima of the function $g^{b_j}_i(\alpha)$.

%         \item From \autoref{lm:max-of-continuous}, we know that the max of continuous functions are also continuous. 
%     \end{enumerate}
% \end{assumption}

\begin{lemma} \label{lm:1-dim-single-piece}
    Let $d_\cW = d_\cA = 1$ and $N = 1, M = 0$. Assume that $(\alpha, \boldsymbol{W}) \in [\alpha_{\min}, \alpha_{\max}] \times [W_{\min}, W_{\max}]$. Then for any function $g_x \in \cG$, we have
    \begin{enumerate}[label=(\alph*)]
        \item The hyperparameter domain $\cA$ can be partitioned into at most $\cO(d_p^2)$ intervals such that $g_x$ is a continuous function over any interval in the partition.
        \item $g_x$ has at most $\cO(d_p^3)$ local maxima for any $x$. 
    \end{enumerate} 
\end{lemma}
\proof 
\noindent (a) Denote $h_x(\alpha, W) = \frac{\partial f(\alpha, \boldsymbol{W})}{\partial \boldsymbol{W}}$. From assumption, $f_x(\alpha, \boldsymbol{W})$ is a polynomial of $\alpha$ and $\boldsymbol{W}$, therefore it is differentiable everywhere in the compact domain $[\alpha_{\min}, \alpha_{\max}] \times [W_{\min}, W_{\max}]$. From Fermat's interior extremum theorem, for any $\alpha_0$, $f_x(\alpha_0, \boldsymbol{W})$ attains the local maxima $\boldsymbol{W}$ either in $\boldsymbol{W}_{\min}, \boldsymbol{W}_{\max}$, or for $\boldsymbol{W} \in [W_{\min}, W_{\max}]$ such that $h_x(\alpha_0, W) = 0$. Note that from assumption, $f_x(\alpha, \boldsymbol{W})$ is a polynomial of degree at most $d_p$ in $\alpha$ and $\boldsymbol{W}$. This implies $h_x(\alpha, \boldsymbol{W})$ is a polynomial of degree at most $d_p - 1$. 

Denote $C_x = V(h_x)$ the zero set of $h_x$. For any $\alpha_0$, the curve $C_x$ intersects the line $\alpha = \alpha_0$ in at most $d_p  - 1$ points by Bezout's theorem. This implies that, for any $\alpha$, there are at most $d_p + 1$ candidate values of $\boldsymbol{W}$ which can possibly maximize $f_x(\alpha, \boldsymbol{W})$, which can be either $W_{\min}, W_{\max},$ or in the curve $C_x$. We then define the \textit{candidate arc set} $\cC: \cA \rightarrow \cM_\alpha(C_x)$ as the function that map $\alpha_0 \in \cA$ to the set of all maximal $\alpha$-monotonic arcs of $C_x$ (\autoref{def:monotonic-curve}) that intersect with $\alpha = \alpha_0$. By the argument above, we have $\abs{\cC(\alpha)} \leq d_q + 1$ for any $\alpha$.

We now have the following claims: (1) $\cC$ is a piece-wise constant function, and (2) any point of discontinuity of $g_x$ must be a point of discontinuity of $\cC$. For (1), we will show that $\cC$ is piece-wise constant, with the piece boundaries contained in the set of $\alpha$-extreme points\footnote{An $\alpha$-extreme point of an algebraic curve $C$ is a point $p = (\alpha, W)$ such that there is an open neighborhood $N$ around $p$ for which $p$ has the smallest or largest $\alpha$-coordinate among all points $p' \in N$ on the curve.} of $C_x$. Indeed, for any interval $I = (\alpha_1, \alpha_2) \subseteq \cA$, if there is no $\alpha$-extreme point of $C_x$ in the interval, then the set of arcs $\cC(\alpha)$ is fixed over $I$ by \autoref{def:monotonic-curve}. Next, we will prove (2) via an equivalent statement: assume that $\cC$ is continuous over an interval $I \subseteq \cA$, we want to prove that $g_x$ is also continuous over $I$. Note that if $\cC$ is continuous over $I$, then $g_x(\alpha)$ involves a maximum over a fixed set of $\alpha$-monotonic arcs of $C_x$, and the straight lines $W = W_{\min}$, $W_{\max}$. Since $f_x$ is continuous along these arcs, so is the maximum $g_x$. 

% \red{Q: does the union of those arcs form a connected domain? If not, then the previous argument seems not rigorous. }
% \red{I might missing something here: using the same logic, and knowing that $f_x$ also continuous along $C_x$, does it also imply that $g_x$ is also continuous in the whole domain $\cA$?}

The above claims imply that the number of $\alpha$-extreme point of $C_x$ upper-bounds the number of discontinuity points of $g_x(\alpha)$. Note that $\alpha$-extreme points $C_x$ satisfies the following equalities: $h_x = 0$ and $\frac{\partial h_x}{\partial W} = 0$. By Bezout's theorem and from assumption on the degree of the polynomial $f_x$, we conclude that there are at most $(d_p - 1) (d_p - 2) = \cO(d_p^2)$ $\alpha$-extreme point of $C_x$. 

\noindent (b) Consider any interval $I$ over which the function $g_x(\alpha)$ is continuous. By \autoref{cor:max-local-maxima-condition}, it suffices to bound the number of elements of the set of local maxima of $f_x$ along the algebraic curve $C_x$ and the straight line $W = W_{\min}$, $W_{\max}$. 

To bound the set of bound the number of elements of the set of local maxima of $f_x$ along the algebraic curve $C_x$, consider the Lagrangian
$$
    \cL(\alpha, W, \lambda) = f_x(\alpha, W) + \lambda h_x(\alpha, W).
$$
From Lagrange's multiplier theorem, any local maxima of $f_x$ along the algebraic curve $C_x$ is also the critical point of $\cL$, which satisfies the following equations
\begin{equation*}
    \begin{aligned}
        \frac{\partial \cL}{\partial \alpha} &= \frac{\partial f_x}{\partial \alpha} + \lambda \frac{\partial h_x}{\partial \alpha}, \\
        \frac{\partial \cL}{\partial W} &= \frac{\partial f_x}{\partial W} + \lambda \frac{\partial h_x}{\partial W}, \\
        \frac{\partial \cL}{ \partial \lambda} &= h_x(\alpha, W) = 0.
    \end{aligned}
\end{equation*}
By Bezout's theorem and from assumption on the degree of the polynomial $f_x$, the system of equations above has at most $d_p^2(d_p - 1)$. Similarly, the equation $f_x(\alpha, W_{\min})$ and $f_{x}(\alpha, W_{\lambda})$ also have at most $d_p - 1$ solutions each. Therefore, we conclude that the number of maxima of $g_x$ can be upper-bounded by $\cO(d_p^3)$.  
\qed 
\begin{theorem} \label{thm:1-dim-single-piece}
     $\Pdim(\cG^*) = \cO(\log d_p)$.
\end{theorem}
\proof 
From \autoref{lm:1-dim-single-piece}, we conclude that $g_x$ has at most $\cO(d_p^3)$ oscillations for any $g_x \in \cG$. Therefore, from \autoref{lm:vcdim-oscillation}, we conclude that $\Pdim(\cG^*) = \cO(\log d_p)$. \qed 

\subsection{Third case: one-dimensional parameter and multiple pieces}
We now extend the results of single piece to multiple pieces case. 
\begin{lemma} \label{lm:1-dim-multi-piece}
Let the dimension of both parameter and hyperparameter $d_\cW = d_\cA = 1$. Assume that $(\alpha, W) \in [\alpha_{\min}, \alpha_{\max}] \times [W_{\min}, W_{\max}]$. Recall that $d_p$ and $d_b$ are the maximum degree of piece and boundary functions, respectively. Then for any function $g_x \in \cG$, we have
    \begin{enumerate}[label=(\alph*)]
        \item The hyperparameter domain $\cA$ can be partitioned into at most $\cO(NM(d_p^2 + d_b^2))$ intervals such that $g_x$ is a continuous function over any interval in the partition, where $N$ and $M$ are the upper-bound for the number of piece and boundaries, respectively. 
        \item $g_x$ has at most $\cO(NM(d_b^3 + d_p^3))$ local maxima for any $x$. 
    \end{enumerate} 
\end{lemma}
\proof (a) The high level idea is similar to that of \autoref{lm:1-dim-single-piece}. To begin with, we can rewrite $g(\alpha)$ as 
\begin{equation*}
    g_x(\alpha) = \max_{i \in [N]}\max_{W: (\alpha, W) \in R_i}f_{x, i}(\alpha, W) = \max_{i \in [N]}g_{x, i}(\alpha),
\end{equation*}
where $R_{x, i}$ is the region where $g_x$ admits the form of piece function $f_{x, i}$. See \autoref{sec:prelimiary} for detailed notations and problem settings. We first give an upper-bound for the number of discontinuity points of $g_{x, i}(\alpha)$. 

Denote $B_{x, i} \subseteq B_x$ the set of boundaries that are adjacent to $R_{x, i}$. From Fermat's interior extremum theorem, for any $\alpha_0 \in \cA$, $f_{x, i}(\alpha, W)$ attains its maximum in either $h_{x, i} = \frac{\partial f_{x, i}(\alpha_0, W)}{\partial W } = 0$, or $b_{x, i, j} = \{k_{x, i, j}(\alpha_0, W) = 0\}$ for any $b_{x, i, j} \in B_{x, i}$. From assumption on the degree of piece and boundary functions, we know that $h_{x, i}$ and $k_{x, i, j}$ are polynomials in $\alpha, W$ of degree at most $d_p - 1$ and $d_b$, respectively. 

For any algebraic curve $C \in B_{x, i}$, $C$ intersect the line $\alpha = \alpha_0$ in at most $d_b$ points by Bezout's theorem. This implies that, for any $\alpha$, there are at most $M d_b$ candidate values of $W$, where $(\alpha, W) \in C$. For each $C \in B_{x, i}$, we define the \textit{candidate arc set} $\cC_C: \cA \rightarrow \cM_A(C)$ as the function that maps $\alpha_0 \in \cA$ to the set of all maximal $\alpha$-monotonic arcs of $C$ that intersect with $\alpha = \alpha_0$. Then for any $C \in B_{x, i}$, we have $\abs{\cC_C(\alpha)} \leq d_b$. Similarly, if $C = \{h_{x, i}(\alpha, W) = 0\}$, then we have $\abs{\cC_C(\alpha)} \leq d_p -1$. 

Similar to the proof of Lemma \ref{lm:1-dim-single-piece}, we have the following claim: (1) $\cC_C(\alpha)$ is a piece-wise constant function for any $C \in \{h_{x, i}(\alpha, W) = 0\} \cup B_{x, i}$, (2) Any point of discontinuity of $g_{x, i}$ most be a point of discontinuity of a $\cC_C$ for $C \in \{h_{x, i} = 0\} \cup B_{x, i}$. This implies that, the total number of $\alpha$-extreme points of $C \in \{h_{x, i} = 0\} \cup B_{x, i}$ upper-bounds the number of discontinuity points of $g_{x, i}(\alpha)$. Therefore, the number of discontinuity points of $g_{x, i}(\alpha)$ is upper-bounded by $M d_b(d_b - 1) + (d_p - 1)(d_p - 2)$.

Note that $g_x(\alpha) =  \max_{i \in [N]}g_{x, i}(\alpha)$. From \autoref{lm:max-of-continuous}, we claim that any discontinuity point of $g_x(\alpha)$ is discontinuity point of $g_{x, i}(\alpha)$ for some $i \in [N]$. Therefore, the number of discontinuity point of $g_x(\alpha)$ is upper-bounded by $N(M d_b(d_b - 1) + (d_p - 1)(d_p - 2))$.


\noindent (b) In a continuous interval of $g_x(\alpha)$, similar to the proof of Lemma \ref{lm:1-dim-single-piece}, we claim that any local maxima of $g_x(\alpha)$ is a local maxima of $g_{x, i}(\alpha)$ for some $i \in [N]$. And any local maxima of $g_{x, i}$ is the local maxima of $f_{x, i}$ along one of algebraic curves $C \in \{h_{x, i} = 0\} \cup B_{x, i}$. Along $C = \{h_{x, i} = 0\}$, the number of local maxima of $f_{x, i}$ is upper-bounded by $\cO(d_p^3)$. Along any $C \in B_{x, i}$, the number of local maxima of $f_{x, i}$ is upper-bounded by $\cO(d_b^3)$. Therefore, we conclude that the number of local maxima of $g_x(\alpha)$ is upper-bounded by $\cO(NM(d_b^3 + d_p^3))$.
\qed 
\begin{theorem} \label{thm:multi-dim-single-piece}
     $\Pdim(\cG^*) = \cO(\log NM(d_b^3 + d_p^3))$.
\end{theorem}

\proof From \autoref{thm:multi-dim-multi-piece}, we conclude that $g_{x, i}$ has at most $\cO(NM(d_b^3 + d_p^3))$ oscillations for any $g_{x, i} \in \cG$. Therefore, from \autoref{lm:vcdim-oscillation}, we conclude that $\Pdim(\cG^*) = \cO(\log NM(d_b^3 + d_p^3))$. \qed 

\subsection{Fourth case: high-dimensional parameter, one-dimensional hyperparameter, single piece, with only region constraints}
\paragraph{Problem setting. } In this section, we consider a simple case where the parameter $\boldsymbol{W} = (W_1, \dots, W_{d_\cW})$ is high-dimensional, and the hyper-parameter $\alpha$ is still one-dimensional. Formally, we have $d_\cW = d$ and $d_\cA = 1$, $N = 1$, $M = 0$. We also assume that $\alpha \in [\alpha_{\min}, \alpha_{\max}]$ and $\boldsymbol{W} \in [W_{\min}, W_{\max}]^{d_\cW}$.

\subsubsection{The proof}
\begin{assumption}[Regularity assumptions] \label{asmpn:zero-regular-value}
Let $f_x(\alpha, \boldsymbol{W})$, where $(\alpha, \boldsymbol{W}) \in \bbR^{d_\cW}$ be the piece function. Denote $F: \bbR^{d_\cW + 1} \rightarrow \bbR^{d_\cW}$ the derivative mapping of $f$, where 
$$
    F(\alpha, \boldsymbol{W}) = \left(\frac{\partial f_x (\alpha, \boldsymbol{W})}{\partial W_1}, \dots,\frac{\partial f_x (\alpha, \boldsymbol{W})}{\partial W_{d_\cW}} \right).
$$
Then, we assume that $\boldsymbol{0} \in \bbR^{d_\cW}$ is a regular value of $F$, thus implying that $F^{-1}(\boldsymbol{0})$ is a 1-dimensional submanifold in $\bbR^{d_\cW + 1}$, which can be partitioned into connected 1-dimensional submanifolds. Here, $F^{-1}(0)$ is exactly the algebraic set defined by $V_x = \cap_{i = d}^{d_\cW}\{(\alpha, \boldsymbol{W}) \mid \frac{\partial f(\alpha, \boldsymbol{W})}{\partial W_i} = 0\}$. 
\end{assumption}
The intuitive idea of the assumption is that if we intersecting $k$ hypersurfaces in $\bbR^{d}$ dimension, we should get a $(d - k)$-dimensional hypersurface. In our scenario, the piece function $f(\alpha, W)$ is a polynomial of $\alpha$ and $W$, and so are the partial derivatives $\frac{\partial f}{\partial W_i}$, which implies $F$ is a smooth map. Therefore, \autoref{asmpn:zero-regular-value} is mild, since the set of non-regular value of a smooth map has Lebesgue measure $0$ from \autoref{thm:sard}. Moreover, The following result allows to bound the number of connected 1-submanifolds of $V_x$.
\begin{lemma}[\cite{warren1968lower}] \label{lm:warren-solution-set-connected-component-bound}
If the degree of polynomial $p \in \bbR[x_1, \dots, x_n]$ is $d$, then the number of connected components of $\{\boldsymbol{x} \mid p(\boldsymbol{x}) = 0\}$ does not exceed $2d^n$.
\end{lemma}

We are now ready to give a proof for the main result in this case. 
\begin{lemma} \label{lm:multi-dim-single-piece}
    Let $d_\cA = 1$ and $N = 1, M = 0$. Assume that $(\alpha, W) \in \cD = \cA \times \cW$ where $\cA = [\alpha_{\min}, \alpha_{\max}]$ and $\cW = [W_{\min}, W_{\max}]^{d_\cW}$. For any function $g_x = \max_{W \in \cW}f_x(\alpha, W) \in \cG$, assume that \autoref{asmpn:zero-regular-value} holds. Then
    \begin{enumerate}[label=(\alph*)]
        \item The hyperparameter domain $\cA$ can be partitioned into at most $\cO((d_\cW d_p)^{d_\cW})$ intervals such that $g_x$ is a continuous function over any interval in the partition.
        \item $g_x$ has at most $\cO(d_p(d_pd_\cW)^{2d_\cW})$  local maxima for any $x$. 
    \end{enumerate} 
\end{lemma}
\autoref{lm:multi-dim-single-piece} provides upper-bounds for the number of discontinuous points of the function $g_x(\alpha)$, and its local maxima, which can be converted into the pseudo-dimension upper-bound for the function class $\cG$ via \autoref{lm:vcdim-oscillation}. The idea is to simplify the function $g_x(\alpha)$ as the maximum function over the zero set of partial derivatives and the region boundaries. The zero set of partial derivatives defines a curve in $\bbR^{d_\cW + 1}$, which we can partition into several $\alpha$-monotonic curves and proceed similarly to the 1-dimensional parameter case. The main challenge is to deal with the maximum over the region boundaries, defined by constraints $W_i = W_{\min}$ or $W_i = W_{\max}$. Fortunately, for each equality constraint, we can consider a similar problem, but with a lower parameter dimension, since there is a set of parameters $W_i$ that have fixed values. We then use an induction argument to get the upper-bound for numbers of discontinuity points and local extreme points for $g_x(\alpha)$ in the original problem. The formal proof of \autoref{lm:multi-dim-single-piece} is presented below.

% $\alpha$-monotonic arcs (\autoref{def:monotonic-curve}), which is exactly the value of $f(\alpha, W)$ along those arcs. Note that $f(\alpha, W)$ is continuous in the entire domain. The discontinuity $g_x(\alpha)$ occurs at a point iff the set of $\alpha$-monotonic arcs involves in $g_x(\alpha)$ changes at that point, and the task now is to determine at which points such changes occur. After upper-bounding the number of discontinuity points of $g_x(\alpha)$, we then proceed to upper-bound to the number of its local maxima via upper-bound the number of its extreme points. .

\proof (a) Recall that \blue{$V_x = \cap_{i = d}^{d_\cW}\{(\alpha, W) \mid \frac{\partial f(\alpha, W)}{\partial W_i} = 0\}$} be the algebraic set which is the intersection of the zero sets of the polynomials $\frac{\partial f_x (\alpha, W)}{\partial W_i}$ for $i = 1, \dots, d$, and let $p_x(\alpha, W) = \sum_{i = 1}^{d_\cW}\left(\frac{\partial f(\alpha, W)}{\partial W_i}\right)^2$. Trivially, $V_x = \{(\alpha, W) \mid p_x(\alpha, W) = 0\}$. From the assumption, $f_x$ is a polynomial of degree at most $d_p$. Therefore, $\frac{\partial f_x(\alpha, W)}{\partial W_i}$ is of degree at most $d_p - 1$ in $\alpha$ and $W$, and $p_x$ is a polynomial in $\alpha$ and $W$ of degree at most $2d_p - 2$.  

Since $(\alpha, W) \in [\alpha_{\min}, \alpha_{\max}] \times [W_{\min} \times W_{\max}]^{d_\cW}$ is a compact domain,  from Fermat's interior extremum theorem, for each $\alpha = \alpha_0$, $g(\alpha_0) = \max_{W}f(\alpha_0, W)$ has the extremum $W^*(\alpha_0)$ attained in $V_x$ (meaning that $(\alpha_0, W^*(\alpha_0)) \in V_x$), or in the boundaries defined by $W_i = W_{\min}$ or $W_i = W_{\max}$ (for $i = 1, \dots, d_\cW$). Therefore, we can rewrite $g_x(\alpha)$ as 
$$
    g_{x}(\alpha) = \max\left(\{\max_{W: (\alpha, W) \in V_x}f_x(\alpha, W)\} \cup \bigcup_{i = 1}^{d_\cW}\{\max_{W: W_i = W_{\min}}f_x(\alpha, W)\}\cup \bigcup_{i = 1}^{d_\cW}\{\max_{W: W_i = W_{\max}}f_x(\alpha, W)\}\right).
$$
From \autoref{lm:max-of-continuous}, we know that the discontinuous point of $g_x(\alpha)$ will be the discontinuous point of $h_x(\alpha)$, $k^{1, i}(\alpha)$, and $k^{2, j}(\alpha)$ ($i, j = 1, \dots, d_{\cW}$), where
$$
    h_x(\alpha) = \max_{W:(\alpha, W) \in V_x}f_x(\alpha, W), \quad k^{1, i}_{x}(\alpha) = \max_{W: W_i = W_{\min}}f_x(\alpha, W), \quad k^{2, j}_{x}(\alpha) = \max_{W: W_j = W_{\max}}f_x(\alpha, W).
$$
We now give an upper-bound for the number of discontinuity point of $h_x, k_x^{1, i}$, and $k_x^{2, j}$.  

\begin{enumerate}
    \item Analyze the discontinuity of $h_x$: 
    from \autoref{asmpn:zero-regular-value} and \autoref{lm:preimage-regular-value}, we know that $V_x$ is a 1-manifold of $\bbR^{d_\cW + 1}$. From \autoref{lm:warren-solution-set-connected-component-bound} and note that $V_x = \{(\alpha, W) \mid p_x(\alpha, W) = 0\}$, we know that $V_x$ can be partitioned into at most $2(2(d_p - 1))^{d_\cW + 1}$ connected 1-manifolds. We can further partition each connected 1-manifold to maximal $\alpha$-monotonic arcs (\autoref{def:monotonic-curve}). We note that if $C$ is an $\alpha$-monotonic arc, then $C$ intersects with the hyperplane $\alpha = \alpha_0$ at at most 1 point (\autoref{prop:monotonic-curve-property}), which implies $\max_{W: (\alpha_0, W) \in C)}f(\alpha_0, W) = f(\alpha_0, W^*(\alpha_0))$ where $(\alpha_0, W^*(\alpha_0)) \in C$.

    Denote $\cC_C: [\alpha_{\min}, \alpha_{\max}] \rightarrow \cM_\alpha(C)$ the function that maps $\alpha_0 \in \cA$ to the set $\cC_C(\alpha_0)$ of all maximal $\alpha$-monotonic arcs (\autoref{def:monotonic-curve}) of 1-manifold $C$ that intersects with the hyperplane $\alpha = \alpha_0$. We can see that $\cC_{V_x}(\alpha)$ is a piece-wise constant function, and the discontinuity of $\cC_{V_x}$ either occurs in the $\alpha$-extreme points (\autoref{def:monotonic-curve}) in $V_x$, or in the $\alpha$-end points (\autoref{def:monotonic-curve-end-point}) of each connected 1-manifold $C$. Since there are at most $2(2(d_p - 1))^{d_\cW + 1}$ connected 1-submanifold of $V_x$, the number of $\alpha$-end points is at most $4(2(d_p - 1))^{d_\cW + 1}$.

    It now suffices to bound the number of $\alpha$-extreme points along $V_x$. Note that $\alpha$-extreme points of in $V_x$ is defined by the algebraic set $V_x \cap \{\frac{\partial p_x(\alpha, W)}{\partial \alpha} = 0\}$. Assume that the mapping $F'(\alpha, W)$ admits $\boldsymbol{0}$ as a regular value, where
    $$
        F'(\alpha, W) = \left(\frac{\partial f_x(\alpha, W)}{\partial W_1}, \dots,\frac{\partial f_x(\alpha, W)}{\partial W_{d_\cW}}, \frac{\partial p_x(\alpha, W)}{\partial \alpha} \right),
    $$
    from Bezout's theorem, the number of $\alpha$-extreme point in $V_x$ is at most $(2d_p - 2)(2d_p - 3)$. Therefore, the number of discontinuous point of $\cC_{V_x}$ is at most $4(2(d_p - 1))^{d_\cW + 1} + (2d_p - 2)(2d_p - 3)^{d_\cW}$. Therefore, we conclude that there are at most $4(2(d_p - 1))^{d_\cW + 1} + (2d_p - 2)(2d_p - 3)^{d_\cW}$ discontinuity points of $h_x$.
    
    \item Analyze the discontinuity of $k^{1, i}_x$ and $k^{2, j}_x$: note that both $W_i = W_{\min}$ and $W_{i} = W_{\max}$ define a $d_{\cW}$-dimensional hyperplane boundaries in $\bbR^{d_\cW + 1}$. If $W \in \bbR^{d_\cW}$, we have $2d_\cW$ such boundaries. We can see that the problem of upper-bounding the number of discontinuity point of $k^{t, i}_x$ ($t = 1, 2$) is equivalent to the original problem of \autoref{lm:multi-dim-single-piece}.a, but for with new parameter $\overline{W} = (W_1, \dots, W_{i - 1}, W_{i + 1}, \dots, W_{d_\cW})  \in \bbR^{d_\cW - 1}$ since $W_i$ is fixed. 
    
    Let $b_t$ be the upper-bound for the discontinuity points with $W \in \bbR^{t}$. From the observation above, and from (1), $b_t$ can be described by the following induction
    \begin{equation*}
        \begin{aligned}
            b_1 &= 8(d_p - 1)^2 + (2d_p - 2)(2d_p - 3) = \cO(d_p^2), \\
            b_{t} &= 4(2(d_p - 1))^{t + 1} + (2d_p - 2)(2d_p - 3) + 2t \cdot b_{t - 1} = \cO(d_p^{t + 1} + t b_{t - 1}).
        \end{aligned}
    \end{equation*}
    Here, $b_1$ comes from (1) above. If $W \in \bbR^d$, the upper-bound number of discontinuity points of $g_x(\alpha)$ is equal to the upper-bound $b_t$ for the number of discontinuity in the derivative curve, which is $4(2(d_p - 1))^{t + 1} + (2d_p - 2)(2d_p - 3)$ from (1), plus the one in $2t$ hyperplane boundaries. Giving the upper-bound in each hyperplane boundary is equivalent to solving the original problem but when $W \in \bbR^{t - 1}$. This implies the recursive formulae above. 
    
    To give an upper-bound for $b_t$, notice that
    \begin{equation*}
        \begin{aligned}
            b_t = \cO(d_p^{t + 1} + tb_{t - 1}) &= \cO\left(d_p^{t + 1} + td_p^{t} + \dots + t(t - 1)\dots 2d_p^2\right) = \cO((td_p)^{t}).
        \end{aligned}
    \end{equation*}

    
    % \blue{write down explicitly how I can derive the upper-bound for the serie.}
\end{enumerate}
Combining (1) and (2) above, we conclude that the number of discontinuity points of $g_x(\alpha)$ is $\cO((d_\cW d_p)^{d_\cW})$.
Therefore, $g_x(\alpha)$ can be partitioned into at most $\cO((d_\cW d_p)^{d_\cW})$ intervals such that $g_x$ is a continuous function over any interval in the partition. 

\noindent (b) We now give the upper-bound for the number of local maxima for $g_x$. From (a), it suffices to upper-bound the number of local maxima for $g_x$ in each of its continuous interval. 

Consider an interval $(\alpha_i, \alpha_{i + 1})$ over which $g_x(\alpha)$ is continous. From Fermat's interior extremum theorem, we can write $g_x(\alpha)$ as 
\begin{equation*}
    \begin{aligned}
        g_x(\alpha) = \max \left( \bigcup_{i = 0}^{d_\cW} \bigcup_{j} \bigcup_{k} \{\max_{W}f(\alpha, W) \text{ s.t. }(\alpha, W) \in V_{x, i}^{j, k}\} \right ),
    \end{aligned}
\end{equation*}
Where $V_{x, i}^{j, k}$ is the $k^{th}$ connected component of $j^{th}$ derivative curve in $i$-dimensional boundary. Each $i$-dimensional boundary is defined by the index set $\cI = \{\iota_1, \dots, \iota_i\}$, and a value set $\cV = \{v_1, \dots, v_i\}$, where $v_i \in \{W_{\min}, W_{\max}\}$ defining the hyperplane 
\begin{equation*}
    W_{\iota_1} = v_1, \dots, W_{\iota_i} = v_i.
\end{equation*}
We can see that the number of $i$-dimensional boundaries is $2^{{d_\cW} - i}\frac{{d_\cW}!}{({d_\cW} - i)!}$. 

Each $i$-dimensional boundary $\beta$ (with corresponding index set $\cI_{\beta}$ and value set $\cV_\beta$) defines a derivative curve $V^{j}_{x, i}$, where
$$
V_{x, i}^j = \bigcup_{s \in [{d_\cW}] \setminus \cI_\beta}\{\frac{\partial f(\alpha, \overline{W})}{\partial W_{s}} = 0\}.
$$
Here, $[{d_\cW}] = \{1, \dots, {d_\cW}\}$ and $\overline{W} = (\overline{W}_1, \dots, \overline{W}_{d_\cW})$, where $\overline{W}_{s} = v_s$, for $s \in \cI_\beta$ is a fixed value, and $\overline{W}_t$ remains variable for $t \not \in \cI_\beta$.

Using Lagrangian multiplier, we can conclude that the number of local extrema of $f(\alpha, W)$ over $V_{x, i}^j$ is at most $d_p(2d_p - 1)^{d_\cW + 1}$ for any $i \in [{d_\cW}]$. Therefore, we conclude that the number of local extrema of $g_x(\alpha)$ in each continuous interval is upper-bounded by $B$ , where
\begin{equation*}
    \begin{aligned}
        B &= d_p(2d_p - 1)^{d_\cW + 1} \sum_{i = 0}^{d_\cW}2^{d_\cW - i}\frac{d_\cW!}{(d_\cW - i)!} \\
        &= d_p(2d_p - 1)^{d_\cW + 1} d_\cW! \sum_{i = 0}^{d_\cW}\frac{2^i}{i!} \leq d_p(2d_p - 1)^{d_\cW + 1} d_\cW! e^2 \\
        &\leq d_p(2d_p - 1)^{d_\cW + 1}d_\cW^{d_\cW}e^2 = \cO(d_p(d_pd_\cW)^{d_\cW}).
    \end{aligned}
\end{equation*}
Combining with (a), we conclude that the number of local extrema of $g_x(\alpha)$ is $\cO(d_p(d_pd_\cW)^{2d_\cW})$.
\qed 

\begin{theorem} \label{thm:multi-dim-single-piece-pdim-bound}
     $\Pdim(\cG^*) = \cO(d_\cW\log(d_\cW d_p))$.
\end{theorem}
\proof  From \autoref{lm:multi-dim-single-piece}, we conclude that $g_{x, i}$ has at most $\cO(d_p(d_pd_\cW)^{2d_\cW})$ oscillations for any $g_{x, i} \in \cG$. Therefore, from \autoref{lm:vcdim-oscillation}, we conclude that $\Pdim(\cG^*) = \cO(d_\cW\log(d_\cW d_p))$.
\qed 
